CEG4N: Counter-Example Guided Neural Network Quantization Refinement

Neural networks are essential components of learning-based software systems. However, their high compute, memory, and power requirements make using them in low resources domains challenging. For this reason, neural networks are often quantized before deployment. Existing quantization techniques tend to degrade the network accuracy. We propose Counter-Example Guided Neural Network Quantization Refinement (CEG4N). This technique combines search-based quantization and equivalence verification: the former minimizes the computational requirements, while the latter guarantees that the network's output does not change after quantization. We evaluate CEG4N~on a diverse set of benchmarks, including large and small networks. Our technique successfully quantizes the networks in our evaluation while producing models with up to 72% better accuracy than state-of-the-art techniques.

==> resources/cegio-algorithm.tex <==
\begin{algorithm}[H]
\hspace*{\algorithmicindent} \textbf{Input}: $f$: a neural network represented by a set of layers~\mc{L}; $\mathcal{I}$ a set of inputs where $\mathcal{I}\subseteq\mathbb{R}^{m}$;~\mc{B} a set of bit width choices.\\
\hspace*{\algorithmicindent} \textbf{Output}: \mc{} a set of quantization bit widths following the layer order $\langle~q_1,...,q_L~\rangle$ \\
\begin{algorithmic}[1]
% \STATE $\mathcal{I} \gets \emptyset$\\
\STATE $\mc{B}^\mc{L} \gets \emptyset$\\
\REPEAT 
    \STATE $\mc{B}^\mc{L} _{ga} \gets$ GA($f$, $\mathcal{I}$, \mc{B})\\
    \STATE $\mathcal{I}_{\mathcal{V}} \gets$ VERIFIER($f$, $\mc{B}^\mc{L} _{ga} $) \\
    \STATE $\mathcal{I} \gets \mathcal{I} \cup \mathcal{I}_{V} $\\
    \STATE $\mc{B}^\mc{L} \gets \mc{B}^\mc{L}_{ga}$\\
\UNTIL $\mathcal{I}_{V} == \emptyset$
\end{algorithmic}
\caption{Robust~\nn~quantization following CEGIO setup.\label{alg:rq-cegio}}
\end{algorithm}

==> resources/trash/cegio-algorithm.tex <==
\begin{algorithm}[H]
\hspace*{\algorithmicindent} \textbf{Input}: $f$: a neural network represented by a set of layers~\mc{L}; $\mathcal{I}$ a set of inputs where $\mathcal{I}\subseteq\mathbb{R}^{m}$;~\mc{B} a set of bit width choices.\\
\hspace*{\algorithmicindent} \textbf{Output}: \mc{} a set of quantization bit widths following the layer order $\langle~q_1,...,q_L~\rangle$ \\
\begin{algorithmic}[1]
% \STATE $\mathcal{I} \gets \emptyset$\\
\STATE $\mc{B}^\mc{L} \gets \emptyset$\\
\REPEAT 
    \STATE $\mc{B}^\mc{L} _{ga} \gets$ GA($f$, $\mathcal{I}$, \mc{B})\\
    \STATE $\mathcal{I}_{\mathcal{V}} \gets$ VERIFIER($f$, $\mc{B}^\mc{L} _{ga} $) \\
    \STATE $\mathcal{I} \gets \mathcal{I} \cup \mathcal{I}_{V} $\\
    \STATE $\mc{B}^\mc{L} \gets \mc{B}^\mc{L}_{ga}$\\
\UNTIL $\mathcal{I}_{V} == \emptyset$
\end{algorithmic}
\caption{Robust~\nn~quantization following CEGIO setup.\label{alg:rq-cegio}}
\end{algorithm}

==> sections/related-works.tex <==
%-------------------------------------------
\section{Related Works}
\label{sec:RelatedWorks}
%-------------------------------------------

%\textcolor{orange}{Either completely remove the related works (keep them for your thesis/next paper), or turn them into an appendix.}
\subsection{\nn~Equivalence}
% Paulsen et al.~\cite{Paulsen2020ReluDiff} proposed ReluDiff a differential verification framework to check the equivalence of two similar NNs. Being 1) an original model and 2) its quantized version. This approach relies on symbolic interval propagation and is comprised of two steps: a forward pass and a backward pass. In the forward pass, an over-approximated value differences of corresponding pairs of neurons in the two networks are computed and propagated, layer by layer from the input to the output. If output region is within a region [$-\epsilon, \epsilon$], the property is verified. Otherwise, a fixed umber of concrete examples are sampled from the input space and tests are performed to check if they violate the property. The forward pass is quite conservative an can have implications in efficiency and accuracy. To overcome that, Paulsen et al.~\cite{Paulsen2020NeuroDiff} proposed NeuroDiff, a new symbolic and fine-grained approximation technique that was able to increase both accuracy and efficiency of differential verification. NeuroDiff has mainly to contributions compared to ReluDiff. First, it employs a fine-grained approximation technique for bounding the output difference of neurons for the whole input domain. It is defined as convex approximations, which is able to improve the concretizations used by ReluDiff. The second contribution is the introduction of symbolic variables to represent neurons in hidden layers to overcome the accumulation of approximation errors.
B\"uning et al.~\cite{BuningKS20Equivalence} defined the notion of relaxed equivalence properties that extends the previous notion of equivalence. Arguing that, exact equivalence is hard to fulfill for two NNs, they instead opt to encode the equivalence properties in MILP using the big-M encoding. First, the input domain is restricted to radii around a point in the input space. This restricts the input domain to smaller subsets, for which equality is more likely. Secondly, the output is relaxed to a less strict relation. Instead of requiring that the neural networks have the same output in order to satisfy the equivalence property, two NNs $\mathbf{R}$ and $\mathbf{T}$ are considered equivalent if the classification result of $\mathbf{R}$ is amongst the top-K largest results of $\mathbf{T}$. This work has recently been extended and improved by Teuber et al.~\cite{Teuber2021Equiv}.

More recently Eleftheriadis et al.~\cite{Eleftheriadis2022OnNN} proposed a \nn~equivalence checking technique that is very close to ours. In their work is proposed a technique to encoding \nn~as SMT formulas (e.g., they encode input variables, input constraints, affine transformations, ReLU activations, and the equivalence properties). They use the SMT solver Z3 to check the satisfiability of all formulas. One difference between their work and RC-CEGIO is that RC-CEGIO considered a very strict definition of Top-1-Equivalence, while their technique allows a more relaxed definition of equivalence. But the major difference is that we encode the \ns~as a C program, and not pure SMT formulas.

\subsection{\nn~Quantization}
The quantization performed by RC-CEGIO can be classified as Post-Training Quantization (PTQ), a kind of quantization that adjust weights, bias and activations without retraining or repairing the quantized \ns. PTQ has an advantage over other types of quantizations for requiring minimal amounts of training data, working well when the data is limited or unlabeled~\cite{Gholami2022ASO}. However, PTQ often show considerable accuracy degradation. \nn~quantization can be further classified into Simulated or Integer-only Quantization~\cite{Gholami2022ASO}. In simulated quantization the \nn~parameters are stored in low precision representation but the operation (e.g., matrix multiplication) are conducted in double/floating point arithmetic. While in Integer-only quantization all operations are conducted in integer arithmetic. In that regard, RC-CEGIO can be further classified as simulated quantization. One disadvantage of simulated quantization is that it does not benefit from the fast and efficient low-precision arithmetic.




